Inclusive Jet Longitudinal Double-spin Asymmetry $A_{LL}$ Measurements in 510 GeV Polarized $pp$ Collisions at STAR

In this analysis, I perform the first ever measurement of \(A_{LL}\) for inclusive jet production in \(pp\) collisions at the higher beam energy of \(\sqrt{s}\) = 510 GeV, based on data that STAR recorded during 2012. The higher beam energy extends the sensitivity to gluon polarization down to \(x \sim 0.02\). The high statistics of the data set and the small size of the physics asymmetries, compared to the previous measurements at 200 GeV, required the development of several new or improved analysis procedures in order to minimize the systematic uncertainties. These include: the first implementation by STAR of an underlying event subtraction during jet reconstruction, a much improved technique to estimate the trigger and reconstruction bias effects, a detailed optimization of the PYTHIA tune that provides a much better match between the experimental data and simulated Monte Carlo events, and a new procedure to estimate the uncertainties associated with the PYTHIA tune parameters. The results for inclusive jet \(A_{LL}\) \textit{vs}.\@ jet \(p_T\) in 510 GeV \(pp\) collisions are presented. They are found to be consistent with predictions from recent global analyses of the polarized PDFs that included prior RHIC data in the fit. They are also consistent with the previous STAR inclusive jet \(A_{LL}\) measurements at \(\sqrt{s}\) = 200 GeV in the region where the kinematics for the two beam energies overlap. These results will provide important new constraints on the gluon polarization in the proton in the \(x\) region below that sampled in 200 GeV \(pp\) collisions.

==> appendices.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2012.  
%  For more info about this template or the 
%  TAMU LaTeX User's Group, see http://www.howdy.me/.
%
%  Author: Wendy Lynn Turner 
%	 Version 1.0 
%  Last updated 8/5/2012
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{appendices}
\titleformat{\chapter}{\centering\normalsize}{APPENDIX \thechapter}{0em}{\vskip .5\baselineskip\centering}
\renewcommand{\appendixname}{APPENDIX}

\input{appendix1}
\input{appendix2}

\end{appendices}

==> figures_ch6.tex <==
\begin{figure}[H]
\centering
\includegraphics[scale=0.6]{figures/false_asymmetry_v0.png}
\caption{Falses asymmetries measured in the data before (black) and after (red) the underlying event correction.}
\label{fig:falseasym}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[scale=0.6]{figures/ue_dpt_v0.png}
\caption{Underlying event $dp_T$ in each jet $p_T$ bin before and after the underlying event correction.}
\label{fig:uedpt}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[scale=0.6]{figures/ue_asymmetry_v0.png}
\caption{Underlying event $dp_T$ asymmetry measured in the data with a $p0$ fit in each jet $p_T$ bin after the jet $p_T$ corrected from the underlying events.}
\label{fig:uedpt}
\end{figure}

\begin{table}[H]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
$p_T$ & model corr. & model error & stat.  & total \\
\hline
(6.0, 7.0) & -9.3e-05 & 2e-05 & 7.4e-05 & 7.7e-05 \\
\hline
(7.0, 8.2) & 5.4e-05 & 9.6e-05 & 9.9e-05 & 0.00014 \\
\hline
(8.2, 9.6) & -0.00021 & 7.6e-06 & 0.00011 & 0.00011 \\
\hline
(9.6, 11.2) & -0.00014 & 6.8e-06 & 8.3e-05 & 8.3e-05 \\
\hline
(11.2, 13.1) & -0.00024 & 8.6e-06 & 0.00014 & 0.00014 \\
\hline
(13.1, 15.3) & -0.00026 & 8.8e-06 & 0.00012 & 0.00012 \\
\hline
(15.3, 17.9) & -0.00033 & 1.1e-05 & 0.00019 & 0.00019 \\
\hline
(17.9, 20.9) & -0.00026 & 1.9e-05 & 0.00023 & 0.00023 \\
\hline
(20.9, 24.5) & -0.00041 & 1.4e-05 & 0.0002 & 0.0002 \\
\hline
(24.5, 28.7) & -0.00032 & 1.9e-05 & 0.00031 & 0.00031 \\
\hline
(28.7, 33.6) & -0.00034 & 2.5e-05 & 0.00034 & 0.00034 \\
\hline
(33.6, 39.3) & -0.00011 & 1.8e-05 & 0.00044 & 0.00044 \\
\hline
(39.3, 46.0) & 0.0005 & 4.7e-05 & 0.00065 & 0.00065 \\
\hline
(46.0, 53.8) & 1.1e-05 & 5.3e-05 & 0.00091 & 0.00091 \\
\hline

\end{tabular}
\caption{Trigger bias and reconstruction uncertainty.}
\label{tab:trgbias}
\end{table}

\begin{table}[H]
\centering
\rotatebox{90}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
$p_T$ & $p_T$ shift syst. & BEMC track & BEMC neutral & syst. 7\% track loss & UE syst. & Total \\
\hline
(6.0, 7.0) & 0.085 & 0.098 & 0.15 & -0.0041 & -0.016 & 0.2 \\
\hline
(7.0, 8.2) & 0.085 & 0.12 & 0.16 & -0.21 & -0.0013 & 0.31 \\
\hline
(8.2, 9.6) & 0.097 & 0.14 & 0.2 & -0.24 & -0.019 & 0.36 \\
\hline
(9.6, 11.2) & 0.053 & 0.17 & 0.22 & -0.13 & -0.044 & 0.32 \\
\hline
(11.2, 13.1) & 0.081 & 0.22 & 0.24 & -0.26 & -0.044 & 0.42 \\
\hline
(13.1, 15.3) & 0.045 & 0.27 & 0.26 & -0.26 & -0.07 & 0.46 \\
\hline
(15.3, 17.9) & 0.059 & 0.27 & 0.36 & -0.28 & -0.11 & 0.54 \\
\hline
(17.9, 20.9) & 0.055 & 0.31 & 0.42 & -0.35 & -0.11 & 0.64 \\
\hline
(20.9, 24.5) & 0.051 & 0.38 & 0.47 & -0.41 & -0.11 & 0.74 \\
\hline
(24.5, 28.7) & 0.06 & 0.48 & 0.52 & -0.49 & -0.13 & 0.87 \\
\hline
(28.7, 33.6) & 0.064 & 0.59 & 0.57 & -0.53 & -0.12 & 0.98 \\
\hline
(33.6, 39.3) & 0.072 & 0.71 & 0.64 & -0.52 & -0.13 & 1.1 \\
\hline
(39.3, 46.0) & 0.092 & 0.84 & 0.74 & -0.63 & -0.12 & 1.3 \\
\hline
(46.0, 53.8) & 0.12 & 0.99 & 0.85 & -0.64 & -0.14 & 1.5 \\
\hline
\end{tabular}
}
\caption{jet $p_T$ systematics.}
\label{tab:ptsyst}
\end{table}

\begin{table}[H]
\centering
\begin{tabular}{|c|c|c|}
\hline
$p_T$ & UE syst. & UE/RL syst. \\
\hline
(6.0, 7.0) & 0.00023 & 0.00033 \\
\hline
(7.0, 8.2) & 0.00019 & 0.0003 \\
\hline
(8.2, 9.6) & 0.00017 & 0.00029 \\
\hline
(9.6, 11.2) & 0.00014 & 0.00027 \\
\hline
(11.2, 13.1) & 0.00013 & 0.00026 \\
\hline
(13.1, 15.3) & 0.00011 & 0.00025 \\
\hline
(15.3, 17.9) & 9.9e-05 & 0.00025 \\
\hline
(17.9, 20.9) & 8.7e-05 & 0.00025 \\
\hline
(20.9, 24.5) & 7.5e-05 & 0.00024 \\
\hline
(24.5, 28.7) & 6.5e-05 & 0.00024 \\
\hline
(28.7, 33.6) & 5.7e-05 & 0.00024 \\
\hline
(33.6, 39.3) & 5e-05 & 0.00024 \\
\hline
(39.3, 46.0) & 4.5e-05 & 0.00023 \\
\hline
(46.0, 53.8) & 4e-05 & 0.00023 \\
\hline
\end{tabular}
\caption{Underlying event and relative luminsoity systematics.}
\label{tab:uerlsyst}
\end{table}

\begin{table}[H]
\centering
\begin{tabular}{|c|c|}
\hline
$p_T$ & $R_t$ \\
\hline
(6.0, 7.0) & 0.58 \\
\hline
(7.0, 8.2) & 0.55 \\
\hline
(8.2, 9.6) & 0.58 \\
\hline
(9.6, 11.2) & 0.54 \\
\hline
(11.2, 13.1) & 0.51 \\
\hline
(13.1, 15.3) & 0.47 \\
\hline
(15.3, 17.9) & 0.55 \\
\hline
(17.9, 20.9) & 0.55 \\
\hline
(20.9, 24.5) & 0.53 \\
\hline
(24.5, 28.7) & 0.5 \\
\hline
(28.7, 33.6) & 0.47 \\
\hline
(33.6, 39.3) & 0.45 \\
\hline
(39.3, 46.0) & 0.45 \\
\hline
(46.0, 53.8) & 0.44 \\
\hline
\end{tabular}
\caption{Averaged $R_t$ for each jet $p_T$ bin.}
\label{tab:run12rt}
\end{table}

\begin{table}[H]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
$p_T$ & $<p_T>$ & $p_T$ shift & jet $p_T$ \\
\hline
(6.0, 7.0) & 6.48 & 0.24 & 6.72 \\
\hline
(7.0, 8.2) & 7.56 & 0.12 & 7.68 \\
\hline
(8.2, 9.6) & 8.86 & 0.64 & 9.51 \\
\hline
(9.6, 11.2) & 10.35 & 1.11 & 11.46 \\
\hline
(11.2, 13.1) & 12.07 & 1.08 & 13.15 \\
\hline
(13.1, 15.3) & 14.09 & 1.47 & 15.56 \\
\hline
(15.3, 17.9) & 16.52 & 2.43 & 18.94 \\
\hline
(17.9, 20.9) & 19.28 & 2.85 & 22.14 \\
\hline
(20.9, 24.5) & 22.52 & 3.13 & 25.66 \\
\hline
(24.5, 28.7) & 26.36 & 3.35 & 29.70 \\
\hline
(28.7, 33.6) & 30.81 & 3.63 & 34.45 \\
\hline
(33.6, 39.3) & 36.00 & 3.70 & 39.71 \\
\hline
(39.3, 46.0) & 42.06 & 4.15 & 46.21 \\
\hline
(46.0, 53.8) & 49.14 & 4.55 & 53.69 \\
\hline

\end{tabular}

\caption{Average jet $p_T$ and the $p_T$ shift for each jet $p_T$ bin.}
\label{tab:run12rt}
\end{table}

==> nomenclature.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2012.  
%  For more info about this template or the 
%  TAMU LaTeX User's Group, see http://www.howdy.me/.
%
%  Author: Wendy Lynn Turner 
%	 Version 1.0 
%  Last updated 8/5/2012
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           NOMENCLATURE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter*{NOMENCLATURE}
\addcontentsline{toc}{chapter}{NOMENCLATURE}  % Needs to be set to part, so the TOC doesnt add 'CHAPTER ' prefix in the TOC.

\begin{tabular}{ll}
B/CS  & Bryan/College Station\tabularnewline
HSUS & Humane Society of the United States\tabularnewline
P & Pressure\tabularnewline
T  & Time\tabularnewline
TVA & Tennessee Valley Authority\tabularnewline
TxDOT \hfill{}\hfill{}\hfill{}\hfill{}\hfill{}\hfill{}\hfill{}\hfill{} & \multicolumn{1}{l}{Texas Department of Transportation}\tabularnewline
\end{tabular}

\vspace{2em}

This page is optional.

\pagebreak{}
